Aligning component upgrades

Modern software systems, like GNU/Linux distributions or Eclipse-based development environment, are often deployed by selecting components out of large component repositories. Maintaining such software systems by performing component upgrades is a complex task, and the users need to have an expressive preferences language at their disposal to specify the kind of upgrades they are interested in. Recent research has shown that it is possible to develop solvers that handle preferences expressed as a combination of a few basic criteria used in the MISC competition, ranging from the number of new components to the freshness of the final configuration. In this work we introduce a set of new criteria that allow the users to specify their preferences for solutions with components aligned to the same upstream sources, provide an efficient encoding and report on the experimental results that prove that optimising these alignment criteria is a tractable problem in practice.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{C. Drescher, I. Lynce and R. Treinen (eds.):\\ Workshop on Logics for Component Configuration (LoCoCo 2011)\\
EPTCS 65, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.65.1}{10.4204/EPTCS.65.1}}
\pdfoutput=1

